Intent-aligned AI systems deplete human agency: the need for agency foundations research in AI safety

The rapid advancement of artificial intelligence (AI) systems suggests that artificial general intelligence (AGI) systems may soon arrive. Many researchers are concerned that AIs and AGIs will harm humans via intentional misuse (AI-misuse) or through accidents (AI-accidents). In respect of AI-accidents, there is an increasing effort focused on developing algorithms and paradigms that ensure AI systems are aligned to what humans intend, e.g. AI systems that yield actions or recommendations that humans might judge as consistent with their intentions and goals. Here we argue that alignment to human intent is insufficient for safe AI systems and that preservation of long-term agency of humans may be a more robust standard, and one that needs to be separated explicitly and a priori during optimization. We argue that AI systems can reshape human intention and discuss the lack of biological and psychological mechanisms that protect humans from loss of agency. We provide the first formal definition of agency-preserving AI-human interactions which focuses on forward-looking agency evaluations and argue that AI systems - not humans - must be increasingly tasked with making these evaluations. We show how agency loss can occur in simple environments containing embedded agents that use temporal-difference learning to make action recommendations. Finally, we propose a new area of research called "agency foundations" and pose four initial topics designed to improve our understanding of agency in AI-human interactions: benevolent game theory, algorithmic foundations of human rights, mechanistic interpretability of agency representation in neural-networks and reinforcement learning from internal states.

==> sections/multi_disciplinary_agency.tex <==

What is agency and why should we care about it in the context of AI-safety? We suggest that agency is one of the most important aspects of human life. It is the essential question of causality in human action: how does biology, society, reasoning and other forces interact in our bodies and minds to give rise to human actions? On one hand, agency can be defined simply as the \ul{experience or feeling} that we control our own actions and that we can cause events to occur in the external world (Frith 2013). On the other, it is the much more complex question of \ul{causality}: e.g. do our conscious thoughts or intentions cause actions and whether other forces (biological, social etc) causally affect action? In our view, research into causality of human actions is still in its infancy - but overall points to human actions as highly affected by non-conscious factors (see discussion in this section below). And, more related to AI-safety, we argue that feeling of agency (i.e. being in control) has already been shown to be empirically manipulable and more attention needs to be paid to this pathway by which AI technologies can be intentionally used or can accidentally develop towards harming humans. 

In order to understand the agency-harm failure mode for AI systems we begin with a brief and somewhat selective, introduction to the topic of agency. We selected to present ideas from humanities and science that have reached a consensus or a relative stalemate for a  period of time (i.e. we did not seek to present the latest work on agency without a good reason). In reading these summaries, it is helpful to think whether they are "causal" descriptions: i.e., do they seek to explain the factors that affect decisions and free action; or "phenomenal" descriptions: i.e. do they seek to explain the "feeling" of freedom in decision making.

\begin{itemize}

\item{\textit{Philosophy}. In philosophy, agency falls within the philosophy of action (or action theory) and largely discuss processes underlying willful or intentional actions in humans [cite]. Many discussions on agency overlap with (or are identical to) debates on “free will” which generally focus on \textit{the extent of which human actions are caused - or controlled - by conscious processes rather than being caused by a chain of physical processes ranging all the way down to the subatomic world} [cite history of phil of free will article]. Philosophical opinions fall into two broad groups: (i) incompatibilists who view human actions and intentions as either completely determined by external physical “forces” with consciousness, intention or even reasoning playing no role (determinists) [cite] - and those who largely agree but view random noise as playing a causal role in the selection of actions and goals (libertarians) [cite]; and (ii) compatibilists which view the role of reasoning (in particular) as playing some causal role in action and goal selection [cite]. It should be noted that approximately 60$\%$ of professional philosophers hold a compatibilist view\footnote{https://survey2020.philpeople.org/survey/results/4838}. In keeping with the consensus position on the philosophy of agency, we  summarize the philosophical position as follows: \ul{agency is a capacity of humans to select goals and actions by the use of reasons rather than acting reflexively and without being coerced or manipulated by other forces - including biological needs, physical forces or social factors}.}

\item{\textit{Sociology}. Sociologists define agency not as the independence of the individual from external forces, but the individual’s ability to act as a subject within a context despite the existence of such external forces. The "situated identity" of the individual plays a significant role in how they make choices, and agency is often viewed as a capacity distributed across society and institutions. A good summary is provided by Cole et al 2019:

\begin{quote}
\textit{The core challenge at the center of the field of sociology is understanding the relationship between structure and agency. Structure refers to the complex and interconnected set of social forces, relationships, institutions, and elements of social structure that work together to shape the thought, behavior, experiences, choices, and overall life courses of people. In contrast, agency is the power people have to think for themselves and act in ways that shape their experiences and life trajectories. Agency can take individual and collective forms.} (Cole et al 2019)
\end{quote}

While some sociologists view the individual's idiosyncratic navigation of the social world as granting them the power to have agency and enact change, others view that agency - as the freedom of the individual to choose - is impossible and that an individual's opinions, goals and actions are essentially “an effect of [social] power” - echoing similar arguments made by incompatibilist philosophers but from the point of view of social structure and forces. The postmodernist Michelle Foucault has been credited with much of this sociological or historical conception of agency. A rough summary of his position is that individuals are constructed by society (or social "power" to be more precise) not the other way around.

\begin{quote}
\textit{The individual is not to be conceived as a sort of elementary nucleus, a primitive atom, a multiple and inert material on which power comes to fasten or against which it happens to strike, and in so doing subdues or crushes individuals. In fact, it is already one of the prime effects of power that certain bodies, certain gestures, certain discourses, certain desires, come to be identified and constituted as individuals. The individual, that is, is not the vis-a-vis of power; it is, I believe, one of its prime effects. The individual is an effect of power, and at the same time, or precisely to the extent to which it is that effect, it is the element of its articulation. The individual which power has constituted is at the same time its vehicle.} (Foucault, M. 1977).
\end{quote}

Thus, in this view the choice to “do what one wants (particularly in order to avoid unpleasant death or pain)” (Cole et al 2019) is largely determined by the power of social institutions and the individual's interaction with them. In sum, sociologists view agency as less of an individual capacity, but of the institutions, culture and many other factors that support the individual in navigating the complex social world. Thus, a sociology (or historical discourse) based definition of agency could be as \ul{manifestation of social structure on individual and collective action and their interdependence}. We view this sociological and historical conception of (lack of) agency as an important consideration in the development of standards for safety in AI systems (and discuss these w.r.t. agency loss below). [bit more clarification if needed]}
 
\item{\textit{Psychology}. We propose that the psychology of motivation and in particular the notion of "innate needs" from the work of Deci and Ryan (Deci and Ryan 1985) is a representative position from which to understand agency from a psychological angle. In some ways, psychologists reframe the question of agency as one of motivation: rather than evaluating the role of reasoning or social structures in determination of goals and outcomes - we can study "innate" motivation structures to understand what types of goals we are intrinsically motivated to seek out. Behavioral psychology is in part concerned with the preconditions for - and the experience of - action and Deci and Ryan's Self-Determination-Theory (SDT) suggests that agency is the ability to balance between external forces and innate drives (Deci and Ryan 1985). SDT links "intrinsic motivation"\footnote{This idea has a long history in psychology and stands in contrast with behaviorism, such as Skinner's work, that argues external rewards are the main motivations for behavior and learning. For more on intrinsic rewards, see Deci 1971 which shows in some cases the superiority of intrinsic motivation over external rewards for increased task persistence and goal achievement. } with the feeling of agency as an experience of oneself as the "origin" of an action.

\begin{quote}
\textit{Rather than motivations merely being “driven” by spontaneous instincts, or “caused” by environmental events, in self-regulation models the focus is on how individuals can organize and direct their energies, as well as protect themselves against both external controls and inner impulses that can otherwise drive behavior. 
\newline
...
Richard de Charms (de Charms 1968) extended White’s theorizing on intrinsic motivation in his classic work Personal Causation. Here he agreed with White that persons who are intrinsically motivated feel efficacy and agency. Looking further at the concept of agency using the attributional terminology of Heider (Heider 1958), de Charms argued that people who are intrinsically motivated have an internal perceived locus of causality. They see themselves as self-regulating – or causing their own actions. In contrast, de Charms argued that any factor that detracted people from this feeling of being an “origin,” or that led them to experience an external perceived locus of causality would undermine intrinsic motivation.} (Deci et al 2019).
\end{quote} 

SDT, in particular, identifies three main innate needs that lead to well-being: (i) competence: carrying out acts in the world that are effective at changing the world; (ii) autonomy: being able to select and carry out acts according to self-driven desires; and (iii) relatedness: experiencing belonging and acceptance in social groups.  In sum, self-regulation based theories of motivation suggest that agency is \ul{the capacity to fulfil innate drives leading to well being by selecting actions that decrease the role of counterproductive instincts or environmental forces}. [this is a big vague; a bit more work here]
}

\item{\textit{Neuroscience of sense of agency}. Neuroscience is arguably the best poised field to answer questions surrounding causality and agency. Given access to enough neural and behavior data we could answer the question of whether a decision or a choice was determined by a biological/neural state or by a conscious process\footnote{More specifically, evaluate to what extent neural processes underlying conscious evaluations, or reasoning use, affect the final actions.}? Some have attempted to carry out these types of causality research including the well known "readiness potential" experiments (Kornhubber and Deeke 1965) and updated versions of Benjamin Libet (Libet et al 1983) which arguably show changes in neural activity on order of hundreds of milliseconds or seconds prior to action time and even prior to awareness. However, the neuroscience of \ul{causes} of free action or behavior is still in its early stages with challenges to the interpretation of these experiments (see Schurger et al 2012) and adaptations of these paradigms in non-human animals (e.g. Mitelut et al 2022). In contrast, neuroscience of \ul{sense of agency} (SoA)  seeks to answer questions such as: where in the brain is the sense that we are in control of action selection and intent localized? under what conditions can the sense of agency be a false positive (e.g. feel like caused something that one did not cause)? (see Wegner 2003; Haggard 2008). The most promising theories of SoA suggest that evolved neural circuits that generate the “feeling” of control over actions carry out a "comparison" between our expectation or prediction with what occurs in the world (Wolpert and Kawato 1998; Frith 2000; much more on this is discussed below). This comparison can be carried out subconsciously or even cognitively (Wegner 2003). Critically, we can feel a desire or intention to act that is generated by artificial means such as deep-brain-stimulation (DBS; Fried 1991).   

In sum, neuroscience studies focused on SoA suggest that agency is experienced through neural \ul{systems aimed at identifying self causality in the external world.} but does yet address the direct role of forces on the generation of will and intent. 
}
\end{itemize}

We propose that given the diversity of approaches to understanding causality and agency can be viewed as:

\begin{quote}
\textit{
AGENCY: the capacity of individuals to make choices while experiencing the freedom to balance between social forces and biological drives.
}
\end{quote}

This broad definition captures most of the main notions of agency including: (i) the  importance of the "feeling" of freedom during decision making and action selection; and (ii) the central role of biological needs and social forces while preventing them from dominating the experience of choice. Critically, we note that this definition focuses on the "experience" or feeling that accompanies certain types of actions - and not on whether thought patterns or their neural substrates are "parent-less" nodes in a complex web of causal interactions. Thus, SoA is a type of "proxy" for causality in the real world. 

Below we further link AI safety concerns to the biology of "agency" and review arguments for why AI-technologies should increasingly targeting the experience of agency. To summarize a key component of our argument using the dichotomy of agency as "causality" vs. agency as "experience", we view AI technologies will gain an increasing and unprecedented role in "causing" human actions - while preserving and promoting a false sense of causality locus within individual humans (Fig 3). [MAYBE EXPAND JUST A BIT].
